EXPRES I. HD~3651 an Ideal RV Benchmark

The next generation of exoplanet-hunting spectrographs should deliver up to an order of magnitude improvement in radial velocity precision over the standard 1 m/s state of the art. This advance is critical for enabling the detection of Earth-mass planets around Sun-like stars. New calibration techniques such as laser frequency combs and stabilized etalons ensure that the instrumental stability is well characterized. However, additional sources of error include stellar noise, undetected short-period planets, and telluric contamination. To understand and ultimately mitigate error sources, the contributing terms in the error budget must be isolated to the greatest extent possible. Here, we introduce a new high cadence radial velocity program, the EXPRES 100 Earths program, which aims to identify rocky planets around bright, nearby G and K dwarfs. We also present a benchmark case: the 62-d orbit of a Saturn-mass planet orbiting the chromospherically quiet star, HD 3651. The combination of high eccentricity (0.6) and a moderately long orbital period, ensures significant dynamical clearing of any inner planets. Our Keplerian model for this planetary orbit has a residual RMS of 58 cm/s over a $\sim 6$ month time baseline. By eliminating significant contributors to the radial velocity error budget, HD 3651 serves as a standard for evaluating the long term precision of extreme precision radial velocity (EPRV) programs.

==> Tables/RVs_3651.tex <==
\begin{deluxetable}{ccc}
%\tablenum{1}
%\footnotesize
%\centering
\tablecaption{EXPRES  RVs of HD~3651 
\label{tab:3651vels}}
\tablewidth{0pt}
\tablehead{
\colhead{BJD - 2440000.5} & \colhead{Vel \ms}  & \colhead{Err \ms} }
\decimalcolnumbers
\startdata
    18714.48211009 & -10.090 &   0.329  \\
    18714.49031062 &  -9.811 &   0.334  \\
    18715.47687595 & -11.452 &   0.377  \\
    18715.48546612 & -11.262 &   0.396  \\
    18716.41734766 & -12.623 &   0.311  \\
    18716.42423904 & -13.207 &   0.320  \\
    18720.40850325 & -18.070 &   0.344  \\
    18720.41527139 & -19.051 &   0.354  \\
    18720.42381932 & -18.863 &   0.357  \\
    18763.28637972 &  -1.769 &   0.256  \\
    18763.29714591 &  -1.313 &   0.248  \\
    18764.34535997 &  -2.289 &   0.267  \\
    18764.34943500 &  -2.394 &   0.244  \\
    18771.33854183 &  -6.480 &   0.245  \\
    18771.34271843 &  -5.661 &   0.247  \\
    18780.16132642 & -15.030 &   0.282  \\
    18780.17748121 & -15.154 &   0.256  \\
    18787.21703397 & -20.378 &   0.238  \\
    18787.22274520 & -20.169 &   0.227  \\
    18788.32050907 & -13.954 &   0.215  \\
    18788.32587935 & -13.627 &   0.231  \\
    18790.30862700 &   0.366 &   0.231  \\
    18790.31349479 &   0.046 &   0.238  \\
    18794.32807585 &   9.075 &   0.244  \\
    18794.33173219 &   9.856 &   0.249  \\
    18794.33545025 &   9.805 &   0.260  \\
    18795.31191846 &  10.036 &   0.234  \\
    18795.31796264 &  10.024 &   0.232  \\
    18795.32611353 &   9.578 &   0.235  \\
    18796.17017570 &   9.986 &   0.224  \\
    18796.17382060 &  10.117 &   0.232  \\
    18796.17710951 &   9.538 &   0.229  \\
    18796.18026286 &   9.863 &   0.240  \\
    18797.30046059 &  10.105 &   0.222  \\
    18797.30305442 &  10.387 &   0.241  \\
    18797.30541719 &   9.855 &   0.240  \\
    18797.30790745 &  10.522 &   0.224  \\
    18798.15146239 &   9.172 &   0.223  \\
    18798.15491309 &   9.623 &   0.233  \\
    18798.16143104 &   9.313 &   0.229  \\
    18798.16666244 &   9.379 &   0.222  \\
    18801.13207407 &   8.920 &   0.228  \\
    18801.13461611 &   9.765 &   0.224  \\
    18801.13717422 &   8.931 &   0.232  \\
    18801.13951213 &   9.209 &   0.228  \\
    18852.09856255 &  -0.263 &   0.244  \\
    18852.10460678 &  -0.918 &   0.269  \\
    18852.11130739 &   0.012 &   0.255  \\
    18852.11628248 &   0.165 &   0.263  \\
    18854.06973622 &   9.126 &   0.224  \\
    18854.07404844 &   9.113 &   0.249  \\
    18854.07801345 &   8.164 &   0.237  \\
    18854.08173559 &   9.147 &   0.241  \\
    18876.07840576 &   3.332 &   0.247  \\
    18876.08449556 &   3.393 &   0.249  \\
    18876.09783120 &   3.024 &   0.249  \\
    18876.10462468 &   3.286 &   0.262  \\
    18881.08127973 &   1.091 &   0.251  \\
    18881.08885743 &   1.599 &   0.260  \\
    18881.09716023 &   0.765 &   0.263  \\
    18881.10383063 &   1.144 &   0.253  \\
\enddat&a
\end{deluxetable}

